Fault-Tolerant Consensus in Quantum Networks

Fault-tolerant consensus is about reaching agreement on some of the input values in a limited time by non-faulty autonomous processes, despite of failures of processes or communication medium. This problem is particularly challenging and costly against an adaptive adversary with full information. Bar-Joseph and Ben-Or (PODC'98) were the first who proved an absolute lower bound $\Omega(\sqrt{n/\log n})$ on expected time complexity of consensus in any classic (i.e., randomized or deterministic) message-passing network with $n$ processes succeeding with probability $1$ against such a strong adaptive adversary crashing processes. Seminal work of Ben-Or and Hassidim (STOC'05) broke the $\Omega(\sqrt{n/\log n})$ barrier for consensus in classic (deterministic and randomized) networks by employing quantum computing. They showed an (expected) constant-time quantum algorithm for a linear number of crashes $t<n/3$. In this paper, we improve upon that seminal work by reducing the number of quantum and communication bits to an arbitrarily small polynomial, and even more, to a polylogarithmic number -- though, the latter in the cost of a slightly larger polylogarithmic time (still exponentially smaller than the time lower bound $\Omega(\sqrt{n/\log n})$ for classic computation).

==> podc'23_submission/src/algorithm-full.tex <==
\section{The Analysis of CheapQuantumConsensus Algorithm}
\label{sec:consensus-analysis}

To analyze the \textsc{CheapQuantumConsensus} algorithm we first recall a combinations of lemmas from \cite{Bar-JosephB02}.

\begin{lemma}[Lemmas $4.1, 4.2, 4.3$ in \cite{Bar-JosephB02}]\label{lem:same-b}
If all processes have the same value at the beginning of an iteration of the main while loop, then the algorithm returns the decision after at most two iterations.
\end{lemma}

\remove{
The correctness proof in Theorem 7 is incomplete. The protocol in [6] only tolerates $n/10$ corruption. Moreover, the authors also modifies the protocol in [6]. Thus, the correctness does not directly come from [6]

Response: We apologize for the ambiguity. Since there is a version of [6] that describes a protocol tolerating $t < n$ number of faults we decide to refer rather to this paper than applying a borrowed analysis in our paper. This relates also to the modifications whose influence is discussed in the proof of Theorem 7. Specifically, we show that any output of our quantum coin could be viewed as an output of the regular common coin with non-zero probability. Since the algorithm from [6] works with probability 1, any output of the new quantum coin cannot affect the correctness of the algorithm. However, we understand that these gaps might require more detailed analysis and we will be happy to include the full proof of correctness in the next version of our paper.  

!!!Tutaj nie wiem jak poprawic dowod Theorem 7. Moim zdaniem to jest czytelnie napisane jakie zmiany mamy w algorytmie.!!!

}

\begin{theorem}
\label{thm:consensus-constant-technical}
For any $\epsilon>0$, the \textsc{CheapQuantumConsensus} algorithm 
solves Consensus against $n/3$-adversary in $O\Big(\big(\frac{1}{\epsilon}\big)^{4}\Big)$ rounds in expectation while using $O(n^{3\epsilon})$ qubits and communication bits per process (amortized), whp.
%in expectation.

%For any number of crashes $t < n / 3$, the algorithm \textsc{CheapQuantumConsensus} solves Consensus in $O\Big(\big(\frac{1}{\epsilon}\big)^{4}\Big)$ rounds in expectation and uses $O(n\log^{4}{n})$ qubits and bits in expectation.
\end{theorem}
\begin{proof}
First, we argue for correctness. Compared to the protocol of Bar-Joseph and Ben-Or~\cite{Bar-JosephB02}, which works for an arbitrary number of failures $t\le n$, we changed the method of deriving random coin, c.f., line~\ref{line:quantum-flip}. Observe that even if \textsc{CheapQuantumCoin} fails to meet conditions of $t$-resilient coin flip, it always outputs some bit in every non-faulty processes. Thus, regardless of number of crashes the output could be an output of local coin flips with a non-zero probability. Since Bar-Josephs's and Ben-Or's algorithm works with probability $1$ (see Theorem~3 in~\cite{Bar-JosephB02}), thus \textsc{CheapQuantumConsensus} also achieves correctness with probability $1$.

Next, we estimate the expected number of phases (i.e. the number of iterations of the main while loop). We consider only \emph{good} phases, i.e. phases in which the adversary crashed at most $\frac{1}{10}$ fraction of processes that were correct at the beginning of this iteration. Note, that there can be at most $\frac{1}{3} / \frac{1}{10} < 4$ "bad" phases.
Let $x$ be the number of non-faulty processes at the beginning of some good phase. We consider following cases:
\\ \noindent Case \textit{a)} There exists a process that in this iteration executes line~\ref{line:undecided-one} or line~\ref{line:decided-one}. In this case, all other processes have to execute line~\ref{line:decided-one} or line~\ref{line:quantum-flip}, since the number of ones counted in different processes may differ by $\frac{x}{10}$ at most. All processes that in this iteration execute \textsc{CheapQuantumCoin} will set $b_{p}$ to $1$ with probability $\frac{1}{4}$ at least. What follows, in the next iteration all processes will start with $b_{p}$ set to $1$ and by Lemma~\ref{lem:same-b} the algorithms will decide within two next phases.
\\ \noindent Case \emph{b)} There exists a process that in this phase executes line~\ref{line:undecided-zero} or line~\ref{line:decided-zero}. Similarly to the previous case, we observe that all other processes have to execute line~\ref{line:decided-zero} or line~\ref{line:quantum-flip}, since, again, the number of ones counted in different processes may differ by $\frac{x}{10}$ at most. Therefore the same arguments applies, but know the final decision will be $0$.
\\ \noindent Case \emph{c)} None of processes executes one of lines~\ref{line:decided-one},~\ref{line:undecided-one},~\ref{line:undecided-zero}, or~\ref{line:decided-zero}. Thus, all processes participated in \textsc{CheapQuantumCoin} in line~\ref{line:quantum-flip}. By Theorem~\ref{thm:coin}, with probability at least $\frac{1}{4}$, all processes will set value $b_{p}$ to the same value. Thus, again by applying Lemma~\ref{lem:same-b}, we get that the algorithms will decide within two next phases.

We showed that if good phase happens, then the algorithm terminates within $2$ next iterations with probability at least $\frac{1}{4}$. Since there can be at most $4$ bad iterations, thus we can calculate the expected number of iterations as follows
\[
\E(ITE) = \sum_{i = 4}^{\infty} i \bigg(\frac{1}{4}\bigg)^{i} = O(1)
\ .
\]
Executing a single phase takes $O\Big(\big(\frac{1}{\epsilon}\big)^{4}\Big)$ rounds, which is the round complexity of the \textsc{FastCounting} algorithm and an upper bound of the time complexity of the \textsc{CheapQuantumCoin} algorithm, therefore the algorithm terminates in $O\Big(\big(\frac{1}{\epsilon}\big)^{4}\Big)$ rounds in expectation. Similarly, by taking the upper bounds on the communication complexity of the algorithms \textsc{FastCounting} and \textsc{CheapQuantumCoin} we get that the expected number of amortized communication bits used by the algorithm is $O(n^{3\epsilon})$.
\end{proof}
Finally, let us analyze the modified version of the algorithm \textsc{CheapQuantumConsensus} with the difference that processes use parameters $x := 2, d = \log{n}, \alpha := \log{n}$ in lines~\ref{line:fast-counting} and \ref{line:quantum-flip}.


\begin{theorem}
\label{thm:consensus-polylog-technical}
The modified version of the \textsc{CheapQuantumConsensus} algorithm 
solves Consensus against any adversary in $O(\log^{5}n)$ rounds in expectation while using $O(\log^{8}{n})$ qubits and communication bits per process (amortized), whp.
%in expectation.

%For any number of crashes $t < n / 3$, the algorithm \textsc{CheapQuantumConsensus} solves Consensus in $O\Big(\big(\frac{1}{\epsilon}\big)^{4}\Big)$ rounds in expectation and uses $O(n\log^{4}{n})$ qubits and bits in expectation.
\end{theorem}
\begin{proof}
For the correcntess we argue exactly the same as in the proof of previous Theorem.
We also define good and bad phases, with only this differences that now the number of bad phases is at most $O(\log{n})$, since the adversary has the full power of crashing arbitrary number of processes. This being said we get that, by the very same reasoning, that the expected number of phases is
\[
\E(ITE) = \sum_{i = \log{n}}^{\infty} i \bigg(\frac{1}{4}\bigg)^{i} = \Theta(\log{n})
\ .
\]
By examining the time and bits complexity of the algorithms \textsc{FastCounting} and \textsc{CheapQuantumCoin} with parameters $x = 2, d = \log{n}, \alpha = \log{n}$, we get a single phase lasts $O(\log^{4}{n})$ rounds and contributes $O(n\log^{7}{n})$ bits to the total communication complexity. The latter, after dividing by $n$, gives the sought complexity amortized per process. Thus, the theorem follows.
\end{proof}

==> podc'23_submission/src/auxiliary_results.tex <==
\section{Further Results}
\label{sec:auxiliary}

\remove{
\jo{Reviewer 1: Are propositions 1 and 2 correct? I could not follow the argument. It is written that the adversary crashes any process to which p wants to send a message or who sends a message to p. But then why are you counting more than a single such message and saying that it is at most $o(n)$? If the process is crashed for the first message it wants to send to p then it definitely does not send more. I may be missing something here but it is really hard to understand the arguments.

Our response:
 The sum of probabilities is for fixed p over other processes q (sorry for not being precise), so by contradictory assumption it is o(n) with a constant>0 probability. Hence, there is a pair p,q with all four probabilities $o(1)$, which further leads to violating agreement with probability $1-o(1)$ in some execution (by indistinguishability of some executions by p,q). 
}
}

\begin{lemma}
\label{lem:worst-case-comm}
For any Consensus algorithm there is a strategy of an adaptive adversary under which some process sends $\Omega(n)$ messages with non-zero constant probability.  
\end{lemma}

\begin{proof}
Suppose otherwise.
%
Consider any process $p$ and two executions, in one of them $p$ starts with value $0$ and in the other starts with $1$. In both executions, the adversary fails all processes that want to send a message to $p$ and all to whom $p$ sends a message.
For each pair $(p,q)$, we obtain two probabilities $\alpha(p,q),\beta(p,q)$, of $p$ sending a message to $q$ in the first and the second execution.
The sum of probabilities $\sum_{q \in G} \alpha(p,q) + \beta(p,q)$ is $o(n)$ with constant probability $c > 0$, by contradictory assumption (recall that this sum is for the fixed process $p$).


Repeat the above for every process $p$. This way we obtain a complete weighted graph (by weights $\alpha(\cdot,\cdot)$ and $\beta(\cdot,\cdot)$). Again, by contradictory assumption, the total sum of all weights is $o(n^2)$ with the same constant probability $c > 0$, therefore, because the number of pairs is $n(n-1)$, there is a pair $p,q$ such that
\[
\alpha(p,q)+\alpha(q,p)+\beta(p,q)+\beta(q,p) = o(1)
\ .
\]
Consider an execution $\cE$ in which the adversary crashes all but processes $p,q$ in the very beginning. It assigns value $0$ to $p$ and value $1$ to $q$. It follows that in this execution $p,q$ try to communicate directly with probability $\alpha(p,q)+\beta(q,p) = o(1)$.
With complementary probability, $1-o(1)$, they do not communicate. 
In this case, $p$ cannot distinguish this execution $\cE$ from another execution $\cE_p$ in which all processes start with value $0$ but the adversary crashes all of them but $p$ in the beginning -- hence, by validity condition of consensus, $p$ must decide $0$ in both of these executions.
Similarly, $q$ cannot distinguish the constructed execution $\cE$ from execution $\cE_q$ in which all processes start with value $1$ but the adversary crashes all of them but $q$ in the beginning -- hence, by validity condition of consensus, $q$ must decide $1$ in both of these executions. Both the above facts must hold with probability $1$, as validity is required with probability $1$.
Consequently, in the constructed execution $cE$, $p$ decides $0$ while $q$ decides $1$, with probability $1-o(1)$, which violates agreement condition of consensus. This contradiction concludes the proof of the lemma. 
\end{proof}


Next, we argue that no constant-time Consensus algorithm uses amortized polylogarithmic number of communication bits, per process.
%\dk{??? What about the number of qubits ???}

\begin{lemma}
\label{prop:constant-time}
Any quantum algorithm solving Consensus in expected time $O(1)$ requires a polynomial number of messages per process (amortized), whp.
\end{lemma}

\begin{proof}
Consider a Consensus algorithm working in expected $\tau$ number of rounds, for some $\tau=O(1)$.
By Markov inequality, the algorithm terminates by time $2\tau$ with probability at least $1/2$, for every strategy of the (adaptive) adversary.
We base on the idea in the proof of Lemma~\ref{lem:worst-case-comm}, but we do it for every round $r\le 2\tau$ and for number of sent messages in a round being $r\cdot n^{r/(2\tau)}$. Using recursive argument, we argue that there is a set $A_r$ of at least $\Omega(\frac{n}{r\cdot n^{r/(2\tau)}})$ processes (instead of just a pair of elements as in the proof of Lemma~\ref{lem:worst-case-comm}) that communicate with each other with probability $o(1)$, with already sending $\Omega(n^{(r-1)/(2\tau)})$ messages, amortized per process in this set.
In one of the rounds, however, a constant ($1/(2\tau)$) fraction of alive processes must increase their communication peers by factor of at least $n^{1/\tau}$, because in $\tau$ expected rounds (so also with constant probability) they need to contact $\Omega(n)$ other peers in some executions -- 
%with no communication, 
again, by the same argument as in the proof of Lemma~\ref{lem:worst-case-comm} (i.e., otherwise, we could find a pair of them, assign different values, and enforce decision on them with a constant probability, violating agreement condition). 
In such round, the adversary allows them to send their message without crashes, thus enforcing total number of 
$\Omega(\frac{n}{r\cdot n^{r/(2\tau)}} \cdot n^{(r-1)/(2\tau)} \cdot n^{1/\tau})=\Omega(n^{1+1/(2\tau)})$ messages, i.e., at least $\Omega(n^{1/(2\tau)})$ messages amortized per every process in the system. As this happens with a constant probability, the proof follows.
%
%Consider a slight modification of that strategy:
%in each round $i\le \tau$ of an execution, the modified adversary additionally 
%
\end{proof}


==> podc'23_submission/src/fast-counting-analysis.tex <==
\section{The Analysis of FastCounting algorithm}\label{sec:fast-counting-analysis}
\begin{proof}[Proof of Theorem~\ref{thm:fuzzy-counting}]
Let us first argue for the correctness. If $|\mathcal{P}| = 1$, then the conditional statement in line~\ref{line:base-case} proves the correctness. Next, we proceed by induction. Assume that the correctness is proved for any subset $\mathcal{P}' \subseteq \mathcal{P}$. Therefore, whenever a process $p$ executes a recursive call in line~\ref{line:recursive-counting}, its variable $\texttt{active}_{p}$ is assigned to the number being an estimation of non-faulty active processes in the set $\mathcal{P}_{g}$. Consider now set $\{ \texttt{active}_{p} : p \in \mathcal{P} \}$. This is the set of input messages to the execution of the Gossip algorithm, see line~\ref{line:fast-gossip}. Thus, by Theorem~\ref{thm:fast-gossip}, we get that unless all process from a group $\mathcal{P}_{p}$ crashes, then all other non-faulty processes will have the number $\texttt{active}_{p}$ in their sets $\mathcal{R}$ (line~\ref{line:fast-gossip}). Therefore, the sum returned in line~\ref{line:counting-output} is the actual estimate of the number of all-non faulty processes in the set $\mathcal{P}$, since it can differ from the number of all processes starting the algorithm only by the number of crashed processes.

The bounds on time and communication complexity follows immediately from the bounds on complexity of the Gossip algorithm proposed in Theorem~\ref{thm:fast-gossip} and the fact that depth of the recursion at most $O(\log{n} / \log{x})$.
\end{proof}

==> podc'23_submission/src/intro.tex <==
\section{Introduction}



\remove{Reviewer 1: 
"Second, there are numerous typos and language errors that make reading very hard."

"Also it should be mentioned that the first part of the introduction is almost a copy of the abstract, which is a waste of the reader's time." PROBABLY WE SHOULD REPHRASE IT?
}


\remove{Reviewer 2: The main improvement of this work comes from the graph / gossipping technique, but not the quantum power it self. I think combining the existing tools to achieve the communication-efficient quantum coin is interesting. However, I might not consider it as solving a fundamental difficulty in consensus or quantum computing. (Just to remember that we might want to give better explenation why the problem is important.)
}

{\em Consensus} is about making a common decision among the processes' initial input values in  a limited time by every %non-crashed 
non-faulty
process, despite the faulty behaviour of some of the players. 
% Fault-tolerant {\em consensus} is about reaching agreement on some of the input values in  a limited time by (non-crashed) autonomous processes, despite of failures of processes or communication medium.
Since its introduction by Pease, Shostak and Lamport~\cite{PSL} (JACM'80), who ruled out trivial solutions (such as always deciding on the same bit), fault-tolerant consensus has constantly been among foundation problems in distributed computing. 
%Since then the 
This problem has been studied in synchronous/asynchronous and deterministic/randomized computation models and under various fault-tolerant or adversarial models: Fail-Stop (crashes) and Byzantine, Static and Adaptive, Computationally Bounded and Unbounded Adversaries - just to name a few (see Section~\ref{sec:related} for related work). 

%Bar-Joseph and Ben-Or~\cite{Bar-JosephB98} (PODC'98) were the first who proved an absolute lower bound $\Omega(\sqrt{n/\log n})$  on (expected) time complexity of any classic (i.e., randomized or deterministic) consensus algorithm with $n$ processes that succeeds with probability $1$ against a strong (adaptive) adversary.
%(A few years earlier, a higher linear lower bound was proved by Fisher and Lynch~\cite{FL} but only for deterministic solutions.)
%They also proposed a randomized algorithm matching time complexity, thus proving that random bits improve time complexity by factor $\Theta(\sqrt{n\log n})$.

While the landscape of Consensus problem under the classic model of computation is well-developed, much less is known if we allow for quantum computation. The seminal work of Ben-Or and Hassidim~\cite{Ben-OrH05} (albeit a short 5-pager in STOC'05) broke the $\Omega(\sqrt{n/\log n})$ rounds time barrier for classic computing by employing quantum computing to further use the power of randomization in distributed computing.
They showed an (expected) constant-time quantum algorithm for a linear number of crashes $t<n/3$, however, the algorithm is inefficient in terms of communication bits and, even more importantly, in terms of the number of quantum bits (qubits), as it uses $\Omega(n)$ of them per process. Since then no algorithm has managed to reduce the quantum resources needed to solve Consensus. Because generating, maintaining and sending quantum bits is extremely costly (today's quantum devices use less than 500 qubits), thus the main question of our paper emerges~naturally:

{\em Could the number of qubits be substantially reduced without harming the time complexity?}

\remove{!OLD!
In this paper, we improve upon the seminal work of Ben-Or and Hassidim~\cite{Ben-OrH05} by reducing the number of qubits to an arbitrarily small polynomial, and even more, to a polylogarithmic number -- though, the latter in the cost of a slightly larger polylogarithmic time (still exponentially smaller than the time lower bound $\Omega(\sqrt{n/\log n})$ for classic computation). Our algorithm  is based on two 
%entirely different \dk{efficient implementations of} 
qubit-and-communication efficient algorithmic techniques, which are of their own interest. First technique is a new quantum implementation of a common coin, which in constant time uses an arbitrarily small polynomial number of bits $O(n^{\epsilon})$, amortized per process (for any chosen constant $\epsilon>0$), and results in all non-faulty processes returning the same value with a non-zero (ideally, constant) probability.
Second is a deterministic algorithm for counting, which returns, in constant time, a count of the number of input 1 (or 0, resp.) among the processes, with an error not bigger then the number of failures (which is inevitable, as the 
%algorithm 
non-faulty processes
may not have any clue about the input value of the faulty processes). This indeed generalizes upon the state-of-art bounds for recently introduced {\em Fuzzy counting} of Hajiaghayi, Kowalski and Olkowski~\cite{HKO-STOC-2022} (STOC'22), 
%-- their main tool in reducing 
who used it to reduce
the number of (classical) bits in classic consensus to $O(\sqrt{n})$, while maintaining the almost-optimal round complexity $O(\sqrt{n}\log{n})$. 
%More specifically, 
The deterministic Fuzzy Counting algorithm in~\cite{HKO-STOC-2022} 
works in $O(\log^3 n)$ rounds (using $O(\polylog n)$ amortized communication bits per process). 
%and uses  $O(\polylog n)$ amortized communication bits per process. 
Depending on the choice of meta-parameters, our protocol can achieve the same bounds as in~\cite{HKO-STOC-2022}, but it is also capable of solving {\em Fuzzy Counting} in a constant number of rounds and arbitrarily small polynomial number of bits per process.
}%\jo{!OLD!}

%\vspace*{-3ex}
\Paragraph{Distributed setting.} 
\remove{Reviewer 2: I think this work consider the full information adversary model [7], while it is not mentioned throughout the paper. If we are not in the full information model, then the results are incomparable to [7].}

We consider a quantum synchronous message-passing model (c.f.,~\cite{AW}), consisting of $n$~synchronous processes (also called players), each with common clock (a clock tick is called a round or a step) and unique id from the known set $\cP=[n]=\{1,\ldots,n\}$.  

%
Between any pair of processes we assume the existence of a quantum channel being able to transmit reliable\footnote{%
Messages are not lost nor corrupted while in transit.}
messages caring quantum bits, qubits. For the sake of completeness,  we also augment the model by classic point-to-point channels between any pair of processes.
In each round, a process can send (personalized) quantum and classic messages to any selected subset of other processes.
After {\em multicasting messages}, in the same round
a process {\em receives messages} that were just sent to it by other processes, and performs {\em local computation}, which involves both quantum and classic bits.\footnote{%
Local computation also decides what messages to send in the next round and to whom.}
%
%Messages and local computation may involve random and quantum bits (qubits), c.f., Section~\ref{sec:quantum-prel}.

%\Paragraph{Processes' failures and adversaries.}
Processes are prone to {\em crash failures}, also called {\em fail-stops}. 
%or, more generally, message omissions.
A crashed process permanently stops any activity, including sending and receiving messages.
%%%A process that omits messages can drop any message scheduled to be sent in a round by the protocol run in this process. 
%There is an upper bound $f<n$ on the number of crash failures we want to be able to cope with, which is known to all processes in that it can be a part of code of an algorithm.

We model crashes as incurred by a full-information {\em adversary} (the same as in~\cite{Bar-JosephB98,Ben-OrH05}) that knows the algorithm, the exact pure quantum state (see Section~\ref{sec:quantum-prel}) and the classic state of the system at any point of an execution, and has an unbounded computational power. The adversary decides which processes to fail and when. The adversary 
is also {\em adaptive} -- 
%\jo{if it wants to make a decision in a round, 
it can make a decision on-line based on its current full-knowledge of the system. 
However, the adversary does not know the future computation, which means that it does not know future random bits drawn by processes.
%knows \jo{the exact pure quantum state (see Section~\ref{sec:quantum-prel}), and the classic state of the system,}
%\dk{classic (i.e., non-quantum) part of the states}
%decision 
%of processes in this and all previous rounds 
%and can use the knowledge to its best result.

As for the quantum part, the adversary can apply no quantum operation to the system, but it is aware of all quantum and classic changes of state that the network undergoes. If a process is crashed by the adversary, we assume that its quantum bits are not destroyed (in particular, entangled qubits in other processes do not collapse but maintain their entanglement), however they cannot be used in 
%any 
further~computation.
%, unless it decides to crash the process first.  
%\dk{??? What happens with quantum part of the system corresponding to crashed process | Explained ???}

Failures are {\em not clean} -- when a process crashes when attempting to multicast a message, then some of the recipients may receive the message and some may not; this aspect is controlled by the adversary. 
%and increases its power against the algorithm.
A {\em $t$-adversary} is additionally restricted by the the number of crashed processes being {\em smaller than~$t$}; if $t=n$ then the $n$-adversary is also called an unbounded adversary (note that even in such case, at least one process must survive for consensus to make sense).
Throughout the paper, we will be calling the adversary described above ``adaptive'',~for~short.

\Paragraph{{\em Consensus} problem:} each process $p$ has its own initial 
%input 
value $input_p$ and has to output a (common) decision value, so that the following conditions hold:
{\em validity} -- decision must be on an input value of some process; {\em agreement} --	no two processes decide on different values; and {\em termination} -- each process eventually decides on some value, unless it is faulty.
All those three requirements must hold with probability 1. We focus on {\em binary consensus}, in which initial values are in $\{0,1\}$. 

Correctness and complexity -- in terms of time (the number of rounds needed for all processes to terminate) and the 
%(worst-case) 
number of quantum bits (qubits) and communication bits -- are analyzed and maximized (worst-case) against an adaptive adversary. 


We say that a random event occurs \emph{with high probability}
({\em whp} for short), if its probability could be made $1-\cO(n^{-c})$ for any sufficiently large
positive constant $c$ by linear scaling of parameters. 


\remove{
First, is the Hadamard gate $H^{k}$. When applied on a quantum state $\ket{00\ldots 0}$ of $k$ qubits, it creates an equal superposition of all the possible
states of $k$ qubits. Formally, this works as follows: $H^{k}\ket{00\ldots 0} = \sum_{x} \frac{1}{\sqrt{2^{k}}} \ket{x}$, where $x$ iterates over all possible binary strings of length $k$. Second is the $CNOT$ gate applied on two qubits. If $\ket{x} = \alpha\ket{0} + \beta\ket{1}$ then $CNOT(\ket{x}, \ket{y}) = \alpha\ket{0}\ket{y} + \beta\ket{1}\ket{y}$. Informally, $\ket{x}$ is the control qubit, if it is $\ket{1}$ then the bit-wise operation applies to the qubit $\ket{y}$, otherwise identity is applied to $\ket{y}$. In general, any quantum operation $U$ we know how to implement can be extended to one controlled by an additional qubit. If $\ket{x}$ is the control qubit then the
controlled operation acts like $U$ when $\ket{x} = \ket{1}$ and it acts like identity when $\ket{x} = \ket{0}$.}

==> podc'23_submission/src/overlay-graphs.tex <==
\section{Communication Graphs}
\label{sec:communication-graphs}
%TODO rozdzielić tę sekcję. Notacja do notacji, usunąć Twierdzenie 8, resztę przemycić do sekcji 7 która znajdzie się na końcu sekcji 3

In~\cite{CK-PODC09}, Chlebus, Kowalski and Strojnowski proposed using fault-tolerant compact expanders of degree $O(\log{n})$ as communication graphs. In this section, we restate and generalize their tools in the context of graphs of {\em arbitrary degree} $d$ larger than $\log{n}$, which will be needed in the analysis of tools done in the next sections.

\Paragraph{Desired properties of communication graphs.}
Let $\alpha$, $\beta$, $\delta$, $\gamma$ and~$\ell$ be positive integers and $0< \varepsilon <1$ be a real number.
The following definition extends the notion of a lower bound on a node degree:

\BB
\begin{description}
\item[\em Dense neighborhood:]
For a node $v\in V$, a set $S\subseteq N^{\gamma}_G(v)$  is said to be \emph{$(\gamma,\delta)$-dense-neighborhood for~$v$} if each node in~$S\cap N^{\gamma-1}_G(v)$ has at least $\delta$ neighbors in~$S$.
\end{description}
%	
%	By way of  example, if the node degrees in graph~$G$ are at least $\delta$ each, then the set~$N^{\gamma}_G(v)$ is a $(\gamma,\delta)$-dense-neighborhood for~$v$.
%	In general, when there are no bounds on node degrees in terms of $\delta$, a $(\gamma,\delta)$-dense-neighborhood for some node may not exist.	

%We are interested in the following properties of overlay graphs, defined in~\cite{CK-PODC09}:
\BB
\noindent
We want our overlay graphs to have the following properties, for suitable parameters $\alpha$, $\beta$, $\delta$~and~$\ell$:

\BB
\begin{description}

\B
\item[\em Expansion:]
graph~$G$ is said to be  \emph{$\ell$-expanding}, or to be an \emph{$\ell$-expander}, if any two subsets of~$\ell$ nodes each are connected by an edge.
\B
\item[\em Edge-density:]
graph~$G$ is said to be \emph{$(\ell,\alpha,\beta)$-edge-dense} if, for any set $X\subseteq V$ of \emph{at least} $\ell$ nodes, there are at least $\alpha |X|$ edges internal for~$X$, and for any set $Y\subseteq V$ of \emph{at most} $\ell$ nodes, there are at most $\beta |Y|$ edges internal for~$Y$.
\B			
\item[\em Compactness:]
graph~$G$ is said to be \emph{$(\ell,\varepsilon,\delta)$-compact} if, for any set $B\subseteq V$ of at least $\ell$ nodes, there is a subset $C \subseteq B$ of at least $\varepsilon\ell$ nodes such that 
each node's degree in~$G|_C$ is at least~$\delta$. 
We call any such set~$C$ a \emph{survival set for~$B$}.
\end{description}

\BB
\Paragraph{Existence of communication graphs.}
Let $G(n,p)$ be an Erdős–Rényi random graph
%variable whose value is a graph 
of $n$ nodes, in which each pair of nodes is connected by an edge with probability~$p$, independently over all such pairs.
\begin{theorem}[\cite{CK-PODC09}]
\label{thm:overlay-existence}
For a random graph $G(n, y)$ where $832\log{n} / (n-1) \le y \le 1$ and $n$ is larger than an absolute constant, and any integer $\ell$ satisfying $\ell \ge 130\log{n} / y$, the following properties hold with high probability:   
\\
\emph{(i)} it is $(\ell, \frac{2}{3}y\ell^2, \frac{4}{3}y\ell^2)$-edge-expanding, 
\hspace*{4.8em}
\emph{(ii)} it is $(\ell,\frac{1}{3}y\ell,\frac{2}{3}y\ell)$-edge-dense, 
\\
\emph{(iii)} it is $(16\ell,3/4,\frac{2}{3}y\ell)$-compact,
\hspace*{0.5em}
\emph{(iv)} the degree of each node is between $\frac{19}{20}y(n-1)$ and $\frac{21}{20}y(n-1)$.


\end{theorem}

\remove{
\begin{theorem}
For every $n$ and $d$ such that $(130\lg{n})^2 < d < n - 1$, there exists a graph $G(d)$ of $n$ vertices such that:\\
\emph{(i)} it is $(n / \sqrt{d})$-expanding, 
\hspace*{4.8em}
\emph{(ii)} it is $(16n / \sqrt{d},3/4,\frac{2}{3}\sqrt{d})$-compact, 
\\
\emph{(iii)} it is $(n / \sqrt{d}, \frac{1}{3}\sqrt{d}, \frac{2}{3}\sqrt{d})$-edge-dense
\hspace*{0.5em}
\emph{(iv)} the degree of each node is at most $\frac{21}{20}d$.
\end{theorem}
\begin{proof}
Let us set $y := \frac{d}{n}, \ell := \frac{n}{\sqrt{d}}$. By simple calculations we get that $y$ satisfies $832\log{n} / (n-1) \le y \le 1$ and $\ell$ satisfies $\ell \ge 130\log{n} / y$, where the second inequality exploits also the assumption $d \ge (130\log{n})^{2}$. Thus, by Theorem~\ref{thm:overlay-existance} together with a probabilistic method we get that there exists graph $G(d)$ such that it is: $(n/ \sqrt{d}, \frac{2}{3}n, \frac{4}{3}n)$-edge-expanding, $(n / \sqrt{d}, \frac{1}{3}\sqrt{d}, \frac{2}{3}\sqrt{d})$-edge-dense, $(16n / \sqrt{d}, 3 / 4. \frac{2}{3}\sqrt{d})$-compact, and its degree is at most $\frac{21(n-1)}{20n}d < \frac{21}{20}d$.
\end{proof}
}

%In~\cite{CK-PODC09},
%the existence of specific overlay graphs was proved -- we will use them in Section~\ref{sec:local-signaling-short} as elements of the family $\cG$ of graphs to define a low-communication pattern in procedure Local Signaling. 
%Let $\delta, \gamma, k$ be integers such that $\delta = 24\log n$,  $\gamma = 2\log n$ and $25\delta \le k \le \frac{2n}{3}$. 
%Let $G(n,p)$ be an Erdős–Rényi random graph
%variable whose value is a graph 
%of $n$ nodes, in which each pair of nodes is connected by an edge with probability~$p$, independently over all such pairs.

\remove{
\begin{theorem}[\cite{CK-PODC09}]
	\label{theorem:overlay-graphs-exist}
	%		
	For every $n$ and $k$ such that $25\delta \le k \le \frac{2n}{3}$,
	a random graph 
	$G(n,24\delta/k)$ 
%	$\cR(n,24\delta/k)$ 
	satisfies all the below properties whp:
	
	\emph{(i)} it is $(k/64)$-expanding, 
\hspace*{4.8em}
	\emph{(iii)} it is $(k,3/4,\delta)$-compact, 

	\emph{(ii)} it is $(k/64,\delta/8,\delta/4)$-edge-dense,
\hspace*{0.5em}
	\emph{(iv)} the degree of each node is between $22\frac{n}{k}\delta$ and $26\frac{n}{k}\delta$.
\end{theorem}
}
%We define an {\em overlay graph} $G(n, k, \delta, \gamma)$ as an arbitrary graph of $n$ nodes fulfilling the conditions of Theorem~\ref{theorem:overlay-graphs-exist}.
%Graph $G(n, k, \delta, \gamma)$ can be computed locally (i.e., in a single round) and deterministically by each process.
%Specifically, by Theorem~\ref{theorem:overlay-graphs-exist}, 
%the class of graphs satisfying the four properties (i) - (iv) is large, therefore any deterministic search in the class of $n$-node graphs, applied locally by each process, returns the same overlay graph $G(n, k, \delta, \gamma)$ in all processes.\footnote{%
%Recall that each round contributes~$1$ to the time complexity, no matter of the length of {\em local} computation.}

The next lemma shows that small subgraphs of a graph $G(n ,y)$ enjoys good connectivity properties. Let us define two meta-parameters $\delta = \frac{2}{3}y\ell, \gamma := \log{n} / \log{\delta}$.
\begin{lemma}[\cite{CK-PODC09}]\label{lemma:dense-are-big}		
If a graph $G$ is $(\ell,\frac{1}{3}y\ell,\frac{2}{3}y\ell)$-edge-dense, then any  $(\gamma,\delta)$-dense-neighborhood of a node $v\in V$ has at least $\ell$~nodes.
\end{lemma}

%\begin{lemma}
%\label{lemma:survival-small-diameter}	
%In a graph~$G(d)$ of $n$ nodes is
%$(\frac{k}{64})$-expanding, 
%$(\frac{k}{64},\frac{\delta}{8},\frac{\delta}{4})$-edge-dense
%and $(k,\frac{3}{4},\delta)$-compact, 
%then for any set $B\subseteq V$ of at least $k$ nodes and for any two nodes $v,w$ from set $C$ being a survival set of $B$, the nodes $v,w$ are of distance at most $2\gamma + 1$ in graph $G_{|C}$, for any $\gamma\ge 2\lg n$. 
%\end{lemma}


%\Paragraph{The new property.}

%The key new property of overlay graphs with good expansion, edge-\-density and compactness is that survival sets 
%(see compactness) 
%in such graphs~have~small~diameters.
%\BB




==> podc'23_submission/src/previous-related.tex <==
\subsection{Previous and Related Work}
\label{sec:related}

%TODO mention this paper, both here and if possible in the intro https://dl.acm.org/doi/abs/10.1145/3341302.3342070?casa_token=ds7B5avov_UAAAAA:PJysOaHKVmN9ZJL1gniKgCGBSXOWeaqvKrJizDS243z4FbZ_OZpMADlqqzyLBZ3I40jZq9hFCVvDpA
\paragraph{Consensus in the classic (non-quantum) model.}
%Classic consensus against an {\em adaptive adversary}.}

%Consensus against an adaptive adversary, considered in this paper, has been already known as more expensive than against weaker adversaries.
Bar-Joseph and Ben-Or~\cite{Bar-JosephB98} (see also their extended version~\cite{Bar-JosephB02}) proved a lower bound $O(\frac{\sqrt{n}}{\log{n}})$ on expected time complexity of consensus against an adaptive adversary.
They also complemented it by time-optimal randomized algorithm. 
%to the consensus problem was given by Bar-Joseph and Ben-Or~\cite{Bar-JosephB98}. 
Their algorithm uses expected $O(\frac{n^{3/2}}{\log{n}})$ number of communications bits, amortized per process, which has been recently improved by Hajiaghay, Kowalski and Olkowski~\cite{HKO-STOC-2022} to $O(\sqrt{n})$ (while maintaining the almost-optimal round complexity $O(\sqrt{n}\log{n})$).

Fisher and Lynch~\cite{FL} proved a lower bound $f+1$ on {\em deterministic} consensus with $f$ crashes (that actually occurred, i.e., $f<t$), thus separating deterministic solutions from randomized.
%that deterministic synchronous solution requires $f+1$ rounds if up to~$f$~processes~may~crash.
Regarding communication complexity, Amdur, Weber and Hadzilacos~\cite{AWH} showed that 
%$\Omega(n)$ messages need to be sent by a protocol solving consensus in an eventually synchronous environment in a failure-free execution; hence, 
the amortized number of messages
%communication bits 
per process is at least constant,
even in some failure-free execution.
%
Dwork, Halpern and Waarts~\cite{DHW} found a solution with $\cO(\log n)$ messages per process, but requiring an exponential time, and later Galil, Mayer and Yung~\cite{GMY} developed a message-optimal algorithm working in over-linear $\cO(n^{1+\varepsilon})$ time, for any $0<\varepsilon<1$.
%with $\cO(n)$ messages, thus showing that this amount of messages is optimal.
%The drawback of the latter solution is that it runs in an over-linear $\cO(n^{1+\varepsilon})$ time, for any $0<\varepsilon<1$.
They also improved the communication further to a constant number of communication bits per process,
%$O(n)$ bits, 
but the resulting algorithm was exponential in the number of rounds.
%Galil, Mayer and Yung~\cite{GMY} found an early-stopping solution with $\cO(n+fn^\varepsilon)$ communication complexity, for any $0<\varepsilon<1$.
Chlebus and Kowalski~\cite{CK} showed that consensus can be
solved in  $\cO(f+1)$ time and with $\cO(\log^2 f)$ messages
if only the number $n-f$ of non-faulty processors satisfies $n-f=\Omega(n)$.
It was later improved in~\cite{CK-PODC09} to $O(f+1)$ time and $O(\polylog n)$ number of communication bits.
%The time complexity $f+1$ is optimal for consensus, as shown by Fischer and Lynch~\cite{FL}.
%To summarize, when the number of crashes $f$ could be 
%as large as a fraction of 
%close to $n$, 
%}%
%The best deterministic algorithm, given by Chlebus, Kowalski and Strojnowski in \cite{CK-PODC09}, solves consensus in asymptotically optimal time
%the time complexity of deterministic consensus is 
%$\Theta(n)$ and an amortized number of communication bits per process $O(\polylog n)$.
All the abovementioned communication complexities are amortized~per~process.

\Paragraph{Quantum consensus.} To the best of our knowledge, almost all previous papers on quantum consensus concentrated on assuring feasibility of the problem against strong Byzantine adversaries, %or asynchronous setting, \jo{??for which no classical solution exists??}, 
c.f.,~\cite{Cholvi22,Helm-PODC08,LFZ-Physics19}, or on optimizing time complexity, including the work of Ben-Or and Hassidim~\cite{Ben-OrH05} achieving constant time against an adaptive adversary.
%
Sparse quantum communication has been considered by Chlebus, Kowalski and Strojnowski in~\cite{ChlebusKS10}, but their protocols work correctly only with some probability smaller than $1$ and for a specific number of failures corresponding to the probability of success. Another difference is that they used quantum operations to encode the classical inputs in quantum registers and used it to directly solve consensus. In this paper, we show another, more-efficient approach, in which we first create a quantum, weak global coin and later employ this tool to the state-of-the-art framework of solving consensus based on the common coin.
%with the help of the coin.}
Other distributed computing problems, not necessarily fault-prone, were also analyzed in quantum models, c.f.,~\cite{BT-SIGACT08,TKM-TALG12, van2022framework, WuYao}.
%\dk{??? DO WE WANT E.G. RECENT PODC PAPERS HERE ???}

\Paragraph{More efficient classic randomized solutions against {\em weak adversaries}.}

Whenever weaker oblivious adversaries are considered,
randomness itself occurred to be enough in reducing time complexity to a constant. 
%However, whenever randomness is considered, different types of an adversary generating failures could be considered. 
%Message complexity of consensus was extensively studied before. 
%Amdur, Weber and Hadzilacos~\cite{AWH} showed that $\Omega(n)$ messages need to be sent by a protocol solving consensus in an eventually synchronous environment in a failure-free execution.
Chor, Merritt and Shmoys~\cite{CMS} developed constant-time algorithms for consensus against an {\em oblivious adversary} -- that is, the adversary who knows the algorithm but has to decide which process fails and when before the execution starts.
%
%
Their solution, however, requires a linear number of communication bits per process.
Gilbert and Kowalski~\cite{GK-SODA-10} presented a randomized consensus algorithm that achieves optimal communication complexity of $O(1) $ amortized communication bits per process 
%(amortized) 
while terminating in 
$O(\log n) $ time with high probability (whp for short), as long as the number of crashes $ f < n/2 $. 
%against an oblivious adversary.


\Paragraph{Classic consensus in more demanding models.} 
%and/or Counting (gossip?) ???}

%It was shown that more severe failures or asynchrony %or restricted underlying communication networks, 
%could cause a substantially higher complexity.
Dolev and Reischuk~\cite{DR} and Hadzilacos and Halpern~\cite{HH} proved the $\Omega(f)$ lower bound on the amortized message complexity per process %(amortized) 
of deterministic consensus for {\em omission or (authenticated) Byzantine failures}. 
%
However, under some limitation on the adversary and requiring termination only whp, the sublinear expected communication complexity $O(\sqrt{n}\; \polylog{n})$ per process can be achieved even in case of Byzantine failures, as proved by King and Saia~\cite{KingS11}.
%
Such limitations are apparently necessary
to achieve
subquadratic time complexity for Byzantine failures, c.f., Abraham et al.~\cite{AbrahamCDNP0S19}.
%
{\em Asynchrony} also implies large communication --
Aspnes~\cite{Aspnes-JACM-98} proved a lower bound $\Omega(n/\log^2 n)$ on communication complexity per process. The complexity bounds in this setting have been later improved, c.f.,~\cite{AC,AlistarhAKS18}. 
%\jo{That result has been later improved by Attiya and Censor~\cite{AC}, who obtained a tight bound showing that asynchronous Consensus requires $\Theta\left(n^{2}\right)$ (asynchronous) step complexity.}  
%\dk{??? WASN'T IT LATER IMPROVED BY CENSOR-HILLEL ???}
%Alistarh, Aspnes, King and Saia~\cite{AlistarhAKS18} showed the most efficient up to date consensus algorithm achieving communication complexity $O(n\log{n})$ per process (amortized) if less then $n/2$ processes may fail. 
%which improved upon the previous result $O(n\log^2 {n})$ by Aspnes and Waarts~\cite{AspnesW-SICOMP-96} and is asymptotically almost optimal due to the lower bound $\Omega(n/\log^2 n)$ by .
























\remove{%%%%%%%%%%  START  REMOVE  %%%%%%%%%%%%%%%%%%%%%%

\FFF
\Paragraph{Early work on consensus.}
%\hspace*{-1em}
The \emph{Consensus} problem was introduced by Pease, Shostak and Lamport~\cite{PSL}.
Early work focused on {\em deterministic} solutions.
Fisher, Lynch and Paterson~\cite{FLP} showed that the problem is unsolvable in an asynchronous setting, even 
if one process may fail.
Fisher and Lynch~\cite{FL} showed that a synchronous solution requires $f+1$ rounds if up to~$f$~processes~may~crash.


%\paragraph{Consensus in crash-prone message-passing system.}

The optimal complexity of consensus with crashes is known with respect to the time and the number of messages (or communication bits) when each among these performance metrics is considered separately. 
Amdur, Weber and Hadzilacos~\cite{AWH} showed that 
%$\Omega(n)$ messages need to be sent by a protocol solving consensus in an eventually synchronous environment in a failure-free execution; hence, 
the amortized number of messages
%communication bits 
per process is at least constant,
even in some failure-free execution.
\remove{%
%The lower bound~$\Omega(n)$ on the number of messages clearly holds, c.f.,~\cite{AWH}.
Dwork, Halpern and Waarts~\cite{DHW} found a solution with $\cO(n\log n)$ messages but requiring an exponential time, and later
Galil, Mayer and Yung~\cite{GMY} developed an algorithm with $\cO(n)$ messages, thus showing that this amount of messages is optimal.
The drawback of the latter solution is that it runs in an over-linear $\cO(n^{1+\varepsilon})$ time, for any $0<\varepsilon<1$.
They also improved the communication to $O(n)$ bits, but the resulting algorithm was exponential in the number of rounds.
%Galil, Mayer and Yung~\cite{GMY} found an early-stopping solution with $\cO(n+fn^\varepsilon)$ communication complexity, for any $0<\varepsilon<1$.
Chlebus and Kowalski~\cite{CK} showed that consensus can be
solved in  $\cO(f+1)$ time and with $\cO(n\log^2 f)$ messages
if only the number $n-f$ of non-faulty processors satisfies $n-f=\Omega(n)$.
It was later improved in~\cite{CK-PODC09} to $O(f)$ time and $O(n\; \polylog n)$ number of communication bits.
%The time complexity $f+1$ is optimal for consensus, as shown by Fischer and Lynch~\cite{FL}.
To summarize, when the number of crashes $f$ could be 
%as large as a fraction of 
close to
$n$, 
}%
The best deterministic algorithm, given by Chlebus, Kowalski and Strojnowski in \cite{CK-PODC09}, solves consensus in asymptotically optimal time
%the time complexity of deterministic consensus is 
$\Theta(n)$ and an amortized number of communication bits per process $O(\polylog n)$.

\Paragraph{Efficient randomized solutions against {\em weak adversaries}.}

Randomness proved itself useful to break a linear time barrier for time complexity. 
However, whenever randomness is considered, different types of an adversary generating failures could be considered. 
%Message complexity of consensus was extensively studied before. 
%Amdur, Weber and Hadzilacos~\cite{AWH} showed that $\Omega(n)$ messages need to be sent by a protocol solving consensus in an eventually synchronous environment in a failure-free execution.
Chor, Merritt and Shmoys~\cite{CMS} developed constant-time algorithms for consensus against an {\em oblivious adversary} -- i.e., the adversary who knows the algorithm but has to decide which process fails and when before the execution starts.
%
%
Gilbert and Kowalski~\cite{GK-SODA-10} presented a randomized consensus algorithm that achieves optimal communication complexity, using $ \mathcal{O}(1) $ amortized communication bits per process 
%(amortized) 
and terminates in 
$ \mathcal{O}(\log n) $ time with high probability, tolerating up to $ f < n/2 $ crash failures. 
%against an oblivious adversary.


\Paragraph{Randomized solutions against (strong) {\em adaptive adversary}.}
Consensus against an adaptive adversary, considered in this paper, has been already known as more expensive than against
%comparing to 
weaker adversaries.
The time-optimal randomized solution to the consensus problem was given by Bar-Joseph and Ben-Or~\cite{Bar-JosephB98}. Their algorithm works in $O(\frac{\sqrt{n}}{\log{n}})$ expected time and uses $O(\frac{n^{3/2}}{\log{n}})$ amortized communications bits per process, %(amortized), 
in expectation. 
They also proved 
%the 
optimality of their result with respect to the time complexity, while 
here we substantially improve the communication.


\Paragraph{Beyond synchronous crashes.}
It was shown that more severe failures or asynchrony %or restricted underlying communication networks, 
could cause a substantially higher complexity.
Dolev and Reischuk~\cite{DR} and Hadzilacos and Halpern~\cite{HH} proved the $\Omega(f)$ lower bound on the amortized message complexity per process %(amortized) 
of deterministic consensus for {\em (authenticated) Byzantine failures}. 
%
King and Saia~\cite{KingS11} proved that under some limitation on the adversary and requiring termination only whp, the sublinear expected communication complexity $O(n^{1/2}\polylog{n})$ per process can be achieved even in case of Byzantine failures. 
%
Abraham et al.~\cite{AbrahamCDNP0S19} showed necessity of such limitations 
to achieve
subquadratic time complexity for Byzantine failures.

If {\em asynchrony} occurs, the recent result of Alistarh
%, Aspnes, King and Saia
et al.~\cite{AlistarhAKS18} showed how to obtain almost optimal communication complexity $O(n\log{n})$ per process (amortized) if less then $n/2$ processes may fail, which improved upon the previous result $O(n\log^2 {n})$ by Aspnes and Waarts~\cite{AspnesW-SICOMP-96} and is asymptotically almost optimal due to the lower bound $\Omega(n/\log^2 n)$ by Aspnes~\cite{Aspnes-JACM-98}.
%in message-passing networks. 
%Interestingly, the result in~\cite{AlistarhAKS18} uses different approach, which is focused on reducing the asynchrony side effects rather than providing sparse communications graphs, as in our case.


\Paragraph{Efficient Fault-tolerant Counting} 
was introduced by Hajiaghay, Kowalski and Olkowski~\cite{HKO-STOC-22}.
Gossip was introduced by Chlebus and Kowalski~\cite{CK}.
They developed a deterministic algorithm solving %\emph{Gossip-with-Crashes} 
Gossip
in time $\cO(\log^2 f)$ while using $\cO(\log^2 f)$ amortized messages per process, provided $n-f=\Omega(n)$.
They also showed a lower bound  $\Omega(\frac{\log n}{\log(n\log n)-\log f})$ on the number of rounds
in case $\cO(\polylog n)$ amortized messages are used per process.
%
In a sequence of papers~\cite{CK,GKS,CK-DISC06},
$O(\polylog n)$ message complexity, amortized per process, was obtained for any $f<n$, while keeping the polylogarithmic time complexity.
%improved to  in \cite{CK-DISC06}.
Note however that general Gossip requires $\Omega(n)$ communication bits per process for different rumors, as each process needs to deliver/receive at least one bit to all non-faulty processes.
%
%\JOO{
Randomized gossip 
%in a synchronous systems 
against an adaptive adversary is doable
%in such environment there 
%it is possible to achieve Gossip 
w.h.p. in $O(\log^{2}{n})$ rounds 
using $O(\log^{3}{n})$ communication bits per process, for a constant number of rumors of constant size and for $f < \frac{n}{3}$ processes, c.f.,
Alistarh et al.~\cite{AlistarhGGZ10}.
%even if the failures are adaptive. 
%
%In their protocol processes need to have unique names only, while the assumption that every process knows names of other processes is relaxed.
%A similar technique 
%however 
%extended to any aggregation function calculated on the set of all non-faulty processes beside the accumulating function, 
%and its practical evaluations, 
%was used by Gupta et al.~\cite{GuptaRB01}
%to calculate aggregation~functions.
%}

\Paragraph{Other quantum consensus results.}
\dk{??? SHOULD WE PUT ANY RELATED WORK, MOSTLY ON BYZANTINE ???}

\remove{A graph is said to be \emph{$\ell$-expanding}, or to be an \emph{$\ell$-expander}, if any two subsets of~$\ell$ nodes each are connected by an edge; this notion was first introduced by Pippenger~\cite{Pip}.
	%	Observe that $(\ell,\alpha,\beta)$-edge-expansion implies the $\ell$-expanding property for $\alpha>0$.
	%	In our algorithm we will use $\ell$-expanders for $\ell=n/2^i$ and for $\ell=(2/3)^i n/64$, for $i\ge 1$.
	There exist $\ell$-expanders  of the maximum degree $\cO(\frac{n}{\ell}\log n)$, as can be proved by the probabilistic method; such an argument was first used by Pinsker~\cite{Pin}. 
}

}

==> podc'23_submission/src/quantum-coin-proofs.tex <==
\section{The Analysis of \textsc{CheapQuantumCoin} Algorithm}
\label{sec:coin-analysis}




%\section{Why the approach of Chlebus, Kowalski and Strojnowski for $t < n$ does not work.}
%In paper~\cite{ChlebusKS10}, Chlebus, Kowalski and Strojnowski proposed a quantum algorithm that solves Consensus with probability at least $\frac{1}{2}$ in presence of arbitrary number $t < n$ of crashes. However, we suspect that there might be a flaw in their correctness argument. Using the terminology from their paper, in Lemma~7 they argue that the ticket of every non-faulty process $\p$ is delivered to every other non-faulty processes by the end of stage 3 of their algorithm even if $t < n$ crashes occurred. However, they do not argue how tickets of \textit{faulty} processes influence decisions of non-faulty processes. Usually, solving Consensus requires showing that every faulty processes is aware of the same subset of bits that come from faulty processes. They approach this issue by relaxing correctness condition to hold only with $\frac{1}{2}$ probability. This works well if the adversary can crash at most $\frac{1}{2}n$ all processes. In this case, with probability $\frac{1}{2}$ \textit{the largest} ticket is in possession of non-faulty process and is propagated among all non-faulty processes. However, this is no longer true if we allow arbitrary number of crashes. For instance the adversary can choose random $n - \sqrt{n}$ processes, partition them into $\sqrt{n}$ disjoint groups and crash them in such way that each non-faulty process gets information from different group of crashed processes. In this case, with probability $\frac{1}-\frac{1}{\sqrt{n}}$ the largest ticket will be delivered to only one of the non-faulty processes and the agreement will not hold.
\section{The Analysis of \textsc{FastCounting} Algorithm} %\label{sec:fast-counting-analysis}
Let us restate the theorem we prove in this section.
\begin{theorem}%[Section~\ref{sec:gossip-long}]
For any $2 \le x \le n$ and $\delta, \alpha \in \Omega(n)$, the \textsc{FastCounting} deterministic algorithm solves the 
%\Fuzzy 
fuzzy counting problem in $O\Big(\frac{\log{n}}{\log{x}}\big(\frac{\log{n}}{\log{\alpha}}\big)^{3}\Big)$ rounds, using $O\Big(x\frac{\log{n}}{\log{x}}\big(\frac{\log{n}}{\log{\alpha}}\big)^{4} d\alpha^{2}\log{n}\Big)$ (amortized) bits per process.
\end{theorem}
\begin{proof}
Let us first argue for the correctness. If $|\mathcal{P}| = 1$, then the conditional statement in line~\ref{line:base-case} proves the correctness. Next, we proceed by induction. Assume that the correctness is proved for any subset $\mathcal{P}' \subseteq \mathcal{P}$. Therefore, whenever a process $p$ executes a recursive call in line~\ref{line:recursive-counting}, its variable $\texttt{active}_{p}$ is assigned to the number being an estimation of non-faulty active processes in the set $\mathcal{P}_{g}$. Consider now set $\{ \texttt{active}_{p} : p \in \mathcal{P} \}$. This is the set of input messages to the execution of the Gossip algorithm, see line~\ref{line:fast-gossip}. Thus, by Theorem~\ref{thm:fast-gossip}, we get that unless all process from a group $\mathcal{P}_{p}$ crashes, then all other non-faulty processes will have the number $\texttt{active}_{p}$ in their sets $\mathcal{R}$ (line~\ref{line:fast-gossip}). Therefore, the sum returned in line~\ref{line:counting-output} is the actual estimate of the number of all-non faulty processes in the set $\mathcal{P}$, since it can differ from the number of all processes starting the algorithm only by the number of crashed processes.

The bounds on time and communication complexity follows immediately from the bounds on complexity of the Gossip algorithm proposed in Theorem~\ref{thm:fast-gossip} and the fact that depth of the recursion at most $O(\log{n} / \log{x})$.
\end{proof}

==> src/notation.tex <==
\section{Technical preliminaries}
\label{sec:quantum-prel}

\paragraph{Quantum model of computation.}
We focus on quantum properties relevant to our algorithms. A quantum system operates on qubits. Single qubit can be either in a pure or a mixed state. A pure state is a vector in a $2$-dimensional Hilbert space $\mathcal{H}$, while a mixed state is modelled as a probabilistic distribution over pure states. Similarly, a register consisting of $d$ qubits can also be in a pure or a mixed state. A pure quantum state, denoted $\ket{x}$, is a vector of $2^d$-dimensional Hilbert space $\mathcal{H}^{\otimes d} = \mathcal{H} \otimes \ldots \otimes \mathcal{H}$. Again, a mixed state of larger dimension is viewed a probabilistic distribution over pure states. In our paper, we will operate only on pure states, and we will use only the standard computational basis of the Hilbert space, which consists of vectors $\{\ket{b_{1}\ldots b_{d}} : b_{1}\ldots,b_{d} \in \{0,1\}^{d}\}$, to describe the system. Therefore, any state $\ket{x}$ can be expressed as
$\ket{x} = \sum_{i=0}^{2^{d}-1} \alpha_{i}\ket{i}$,
with the condition that $\sum_{i} |\alpha_{i}|^{2} = 1$, since quantum states can be only normalized vectors. 

Transitions, or equivalently -- changes of states of a quantum system, are given by unitary transformations on the Hilbert space of $d$ qubits. These unitary transformations are called {\em quantum gates}. These operations are exhaustive in the sense that any quantum computation can be expressed as a unitary operator on some Hilbert space. There are small-size sets of quantum gates working on two-dimensional space that are universal --
%such that 
any unitary transformation on a $2^{d}$-dimensional quantum space can be approximated by a finite collection of these universal gates. In our applications, any quantum algorithm computation run by a process requires polynomial 
(in $n$) number of universal~gates.
%size in the number $n$ universal gates.

Finally, an important part of quantum computation 
%there 
is also a quantum measurement. Measurements are performed with respect to a basis of the Hilbert space -- in our case this is always the computational basis. A complete measurement in the computational basis executed on a state $\ket{x} = \sum_{i=0}^{2^d - 1}\alpha_{i}\ket{i}$ leaves the state in one of the basis vectors, $\ket{i}$, for $i \in \{0,1\}^{d}$, with probability~$\alpha_{i}^{2}$. The outcome of the measurement is a classic register of $d$ bits, informing 
%which 
to which vector the state has been transformed. It is also possible to measure only some qubits of the system, which is called a partial measurement. If $A$ describes the subset of qubits that we want to measure and $B$ is the remaining part of the system, then the partial measurement is defined by the set of projectors $\{ \Pi_{i} = \ket{i}_{A}\bra{i}_{A} \otimes I_{B} \ \, | \ \, \mbox{for } i \in \{0, 1\}^{d}\}$.\footnote{Whenever it could be irrelevant, from the context, we may follow the standard notation in quantum computing and skip writing normalizing factors.} In the former, a subscript refers to the part of the system on which the object exists, $I$ denotes the identity function, while $\bra{i}$ is a functional of the dual space to the original Hilbert space (its matrix representation is the conjugate transpose of the matrix representation of $\ket{i}$).
If before the measurement the system was in a state $\ket{x}_{AB}$ then, after the measurement, it is in one of the states $\{ \Pi_{i} \ket{x}_{AB} \ \, | \ \, \mbox{for } i \in \{0, 1\}^{d}\}$, where state $\Pi_{i} \ket{x}_{AB}$ is achieved with probability $\bra{x}_{AB}\Pi_{i} \ket{x}_{AB}$.\footnote{$\Pi_{i} \ket{x}_{AB}$ and $\bra{x}_{AB}\Pi_{i} \ket{x}_{AB}$ are simply linear operations on matrices and vectors.} The reader can find a comprehensive introduction to quantum computing in~\cite{NielsenQuantum}.

\Paragraph{Graph notations.}
Let $G=(V,E)$ denote an undirected graph.
Let $W\subseteq V$ be a set of nodes of~$G$.
We say that an edge $(v,w)$ of $G$ is \emph{internal for~$W$} if $v$ and~$w$ are both in~$W$.
We say that an edge $(v,w)$ of $G$ \emph{connects the sets~$W_1$ and $W_2$},
or \emph{is between $W_1$ and $W_2$}, for any disjoint subsets $W_1$ and~$W_2$ of~$V$, if one of its ends is in~$W_1$ and the other in~$W_2$.
The \emph{subgraph of~$G$ induced by~$W$}, denoted~$G|_W$, is the subgraph of~$G$ containing the nodes in~$W$ and all the edges internal for~$W$ in $G$.
A node adjacent to a node~$v$ is a \emph{neighbor of~$v$} and the set of all the neighbors of a node~$v$ is the \emph{neighborhood of~$v$}.
%The notation 
$N^i_G(W)$ 
%is used to denote 
denotes
the set of all the nodes in~$V$ that are of distance at most~$i$ from some node in~$W$ 
in graph~$G$.
In particular, the (direct) neighborhood of~$v$ is denoted~$N_G(v)=N^1_G(v)$. 

The following combinatorial properties are of utter importance 
%for the correctness of 
in the analysis of
our algorithms.
%\noindent \textit{Expansion:} 
Graph~$G$ is said to be  \emph{$\ell$-expanding}, or to be an \emph{$\ell$-expander}, if any two subsets of~$\ell$ nodes each are connected by an edge.
%\\
%\noindent \textit{Edge-density:}
Graph~$G$ is said to be \emph{$(\ell,\alpha,\beta)$-edge-dense} if, for any set $X\subseteq V$ of \emph{at least} $\ell$ nodes, there are at least $\alpha |X|$ edges internal for~$X$, and for any set $Y\subseteq V$ of \emph{at most} $\ell$ nodes, there are at most $\beta |Y|$ edges internal for~$Y$. 
%\\
%\noindent \textit{Compactness:}
Graph~$G$ is said to be \emph{$(\ell,\varepsilon,\delta)$-compact} if, for any set $B\subseteq V$ of at least $\ell$ nodes, there is a subset $C \subseteq B$ of at least $\varepsilon\ell$ nodes such that 
each node's degree in~$G|_C$ is at least~$\delta$. 
We call any such set~$C$ a \emph{survival set for~$B$}.


==> src/our-results.tex <==
\section{Our Results}
%and New Tools}
In this work, we focus on improving quantum bits' and communication complexities (without harming time complexity) of quantum algorithms  solving Consensus problem with probability 1 against an adaptive full-information adversary capable of causing 
processes' crashes.
We observe that the maximum, per process, number of communication bits in Consensus problem is $\Omega(n)$, therefore one can only hope to improve amortized communication complexity (per process), see Lemma~\ref{lem:worst-case-comm} in Appendix~\ref{sec:auxiliary}.

%Hence, in this work, we concentrate on {\em amortized number of communication bits per process}, defined as the total number of bits sent in messages devided by the number of processes $n$.
%which we lower to arbitrary polynomial (with only a constant overhead on the number of rounds) and further to polylogarithm (with logarithmic overhead on the number of rounds).

Our first main result is a quantum algorithm that solves Consensus (correctness with probability~$1$) in expected constant number of rounds and amortized number of qubits and communication bits per process being an arbitrarily low polynomial. This directly improves, by a  polynomial factor, the result of Ben-Or and Hassidim~\cite{Ben-OrH05}, which required a super-linear number of qubits and communication bits, amortized per process. More precisely, in Section~\ref{sec:consensus-alg} we give an algorithm and in Section~\ref{sec:consensus-analysis}~we~prove the following result (see also its technical counterpart -- Theorem~\ref{thm:consensus-constant-technical}):

\begin{theorem}
\label{thm:constant-rounds-consensus}
For 
%any number of crashes $t < n$ and for 
any $\epsilon>0$, there is an algorithm 
%\textsc{CheapQuantumConsensus} 
solving consensus against an adaptive $n/3$-adversary in expected
%$O(1/\epsilon)$ 
$O(1)$
rounds 
%in expectation 
while using $O(n^{\epsilon})$ qubits and communication bits (amortized) per process,~whp.
%in expectation.
\end{theorem}

Although our algorithm, called {\sc CheapQuantumConsensus}, uses an idea of so called weak global coin analogously to e.g.,~\cite{FM,Ben-OrH05}, ours is based on two entirely different qubit-and-communication efficient algorithmic techniques.
%
First technique is a new quantum implementation of a weak global coin, c.f., Definition~\ref{def:coin}, called {\sc CheapQuantumCoin}. It works in constant, $O\big(\frac{1}{\epsilon}\big)$, time, uses an arbitrarily small polynomial number of bits $O(n^{\epsilon})$, amortized per process (for any chosen constant $\epsilon>0$), and results in all non-faulty processes returning the same value with a non-zero 
%(ideally, constant) 
constant
probability, c.f., Theorem~\ref{thm:coin}.
%
Second is a deterministic algorithm for counting, which returns, 
%within polylogarithmic time and with probability 1, 
in constant time,
a count of the number of input~1 (or 0, resp.) among the processes. The output could be different at different processes, due to failures and a short time for counting, but each of them is a number not smaller than the number of processes with input~1 (0, resp.) at the end of the procedure and not larger than the number of processes with input 1 (0, resp.) in the beginning of the procedure. It uses only an arbitrary small polynomial number of communication bits, amortized per process.
%whp.
%
We give an overview of these two techniques in the next Sections~\ref{sec:quantum-coin} and \ref{sec:counting}, respectively, and their analysis in Sections~\ref{sec:coin-analysis} and \ref{sec:fast-counting-analysis}, respectively. 

Although constant-time algorithms cannot achieve low communication, as we argue in Lemma~\ref{prop:constant-time} in Appendix~\ref{sec:auxiliary}, interestingly, we show that our main algorithm could be re-instantiated in such a way that it uses only a polylogarithmic number of qubits and communication to solve consensus in a slightly (polylogarithmically) larger number of rounds (see Section~\ref{sec:consensus-alg} and Appendix~\ref{sec:consensus-analysis}, and technical counterpart Theorem~\ref{thm:consensus-polylog-technical} for more details):
%for details).

\begin{theorem}
\label{thm:polylogarithmic-consensus}
%For any number of crashes $t < n$, 
There is an algorithm 
%\textsc{CheapQuantumConsensus} 
solving consensus against an unbounded~adaptive adversary in 
polylogarithmic number of
%$O(\log^{5}{n})$ 
rounds, in expectation, while using 
a polylogarithmic number of
%$O(\log^{8}{n})$ 
qubits and communication bits (amortized) per process,~whp.
%in expectation.
\end{theorem}

We believe that the newly developed techniques could be also applied to other types of failures, after failure-specific modifications. For example, although message omission failures require linear amortized communication per process (c.f.,~\cite{HH}), one could still use a small polynomial or even a polylogarithmic number of qubits (together with a linear number of classic communication bits) per process, if qubits are handled according to our techniques while some additional classic communication bits are introduced to handle message omissions. We leave details to follow-up~work.
%\dk{??? ANY OTHER OPEN QUESTIONS? WE DONT HAVE CONCLUSIONS ???}


==> src/overlay-graphs.tex <==
\section{Communication Graphs}
\label{sec:communication-graphs}
%TODO rozdzielić tę sekcję. Notacja do notacji, usunąć Twierdzenie 8, resztę przemycić do sekcji 7 która znajdzie się na końcu sekcji 3

In~\cite{CK-PODC09}, Chlebus, Kowalski and Strojnowski proposed using fault-tolerant compact expanders of degree $O(\log{n})$ as communication graphs. In this section, we restate and generalize their tools in the context of graphs of {\em arbitrary degree} $d$ larger than $\log{n}$, which will be needed in the analysis of tools done in the next sections.

\Paragraph{Desired properties of communication graphs.}
Let $\alpha$, $\beta$, $\delta$, $\gamma$ and~$\ell$ be positive integers and $0< \varepsilon <1$ be a real number.
The following definition extends the notion of a lower bound on a node degree:

\BB
\begin{description}
\item[\em Dense neighborhood:]
For a node $v\in V$, a set $S\subseteq N^{\gamma}_G(v)$  is said to be \emph{$(\gamma,\delta)$-dense-neighborhood for~$v$} if each node in~$S\cap N^{\gamma-1}_G(v)$ has at least $\delta$ neighbors in~$S$.
\end{description}
%	
%	By way of  example, if the node degrees in graph~$G$ are at least $\delta$ each, then the set~$N^{\gamma}_G(v)$ is a $(\gamma,\delta)$-dense-neighborhood for~$v$.
%	In general, when there are no bounds on node degrees in terms of $\delta$, a $(\gamma,\delta)$-dense-neighborhood for some node may not exist.	

%We are interested in the following properties of overlay graphs, defined in~\cite{CK-PODC09}:
\BB
\noindent
We want our overlay graphs to have the following properties, for suitable parameters $\alpha$, $\beta$, $\delta$~and~$\ell$:

\BB
\begin{description}

\B
\item[\em Expansion:]
graph~$G$ is said to be  \emph{$\ell$-expanding}, or to be an \emph{$\ell$-expander}, if any two subsets of~$\ell$ nodes each are connected by an edge.
\B
\item[\em Edge-density:]
graph~$G$ is said to be \emph{$(\ell,\alpha,\beta)$-edge-dense} if, for any set $X\subseteq V$ of \emph{at least} $\ell$ nodes, there are at least $\alpha |X|$ edges internal for~$X$, and for any set $Y\subseteq V$ of \emph{at most} $\ell$ nodes, there are at most $\beta |Y|$ edges internal for~$Y$.
\B			
\item[\em Compactness:]
graph~$G$ is said to be \emph{$(\ell,\varepsilon,\delta)$-compact} if, for any set $B\subseteq V$ of at least $\ell$ nodes, there is a subset $C \subseteq B$ of at least $\varepsilon\ell$ nodes such that 
each node's degree in~$G|_C$ is at least~$\delta$. 
We call any such set~$C$ a \emph{survival set for~$B$}.
\end{description}

\BB
\Paragraph{Existence of communication graphs.}
Let $G(n,p)$ be an Erdős–Rényi random graph
%variable whose value is a graph 
of $n$ nodes, in which each pair of nodes is connected by an edge with probability~$p$, independently over all such pairs.
\begin{theorem}[\cite{CK-PODC09}]
\label{thm:overlay-existence}
For a random graph $G(n, y)$ where $832\log{n} / (n-1) \le y \le 1$ and $n$ is larger than an absolute constant, and any integer $\ell$ satisfying $\ell \ge 130\log{n} / y$, the following properties hold with high probability:   
\\
\emph{(i)} it is $(\ell, \frac{2}{3}y\ell^2, \frac{4}{3}y\ell^2)$-edge-expanding, 
\hspace*{4.8em}
\emph{(ii)} it is $(\ell,\frac{1}{3}y\ell,\frac{2}{3}y\ell)$-edge-dense, 
\\
\emph{(iii)} it is $(16\ell,3/4,\frac{2}{3}y\ell)$-compact,
\hspace*{0.5em}
\emph{(iv)} the degree of each node is between $\frac{19}{20}y(n-1)$ and $\frac{21}{20}y(n-1)$.


\end{theorem}

\remove{
\begin{theorem}
For every $n$ and $d$ such that $(130\lg{n})^2 < d < n - 1$, there exists a graph $G(d)$ of $n$ vertices such that:\\
\emph{(i)} it is $(n / \sqrt{d})$-expanding, 
\hspace*{4.8em}
\emph{(ii)} it is $(16n / \sqrt{d},3/4,\frac{2}{3}\sqrt{d})$-compact, 
\\
\emph{(iii)} it is $(n / \sqrt{d}, \frac{1}{3}\sqrt{d}, \frac{2}{3}\sqrt{d})$-edge-dense
\hspace*{0.5em}
\emph{(iv)} the degree of each node is at most $\frac{21}{20}d$.
\end{theorem}
\begin{proof}
Let us set $y := \frac{d}{n}, \ell := \frac{n}{\sqrt{d}}$. By simple calculations we get that $y$ satisfies $832\log{n} / (n-1) \le y \le 1$ and $\ell$ satisfies $\ell \ge 130\log{n} / y$, where the second inequality exploits also the assumption $d \ge (130\log{n})^{2}$. Thus, by Theorem~\ref{thm:overlay-existance} together with a probabilistic method we get that there exists graph $G(d)$ such that it is: $(n/ \sqrt{d}, \frac{2}{3}n, \frac{4}{3}n)$-edge-expanding, $(n / \sqrt{d}, \frac{1}{3}\sqrt{d}, \frac{2}{3}\sqrt{d})$-edge-dense, $(16n / \sqrt{d}, 3 / 4. \frac{2}{3}\sqrt{d})$-compact, and its degree is at most $\frac{21(n-1)}{20n}d < \frac{21}{20}d$.
\end{proof}
}

%In~\cite{CK-PODC09},
%the existence of specific overlay graphs was proved -- we will use them in Section~\ref{sec:local-signaling-short} as elements of the family $\cG$ of graphs to define a low-communication pattern in procedure Local Signaling. 
%Let $\delta, \gamma, k$ be integers such that $\delta = 24\log n$,  $\gamma = 2\log n$ and $25\delta \le k \le \frac{2n}{3}$. 
%Let $G(n,p)$ be an Erdős–Rényi random graph
%variable whose value is a graph 
%of $n$ nodes, in which each pair of nodes is connected by an edge with probability~$p$, independently over all such pairs.

\remove{
\begin{theorem}[\cite{CK-PODC09}]
	\label{theorem:overlay-graphs-exist}
	%		
	For every $n$ and $k$ such that $25\delta \le k \le \frac{2n}{3}$,
	a random graph 
	$G(n,24\delta/k)$ 
%	$\cR(n,24\delta/k)$ 
	satisfies all the below properties whp:
	
	\emph{(i)} it is $(k/64)$-expanding, 
\hspace*{4.8em}
	\emph{(iii)} it is $(k,3/4,\delta)$-compact, 

	\emph{(ii)} it is $(k/64,\delta/8,\delta/4)$-edge-dense,
\hspace*{0.5em}
	\emph{(iv)} the degree of each node is between $22\frac{n}{k}\delta$ and $26\frac{n}{k}\delta$.
\end{theorem}
}
%We define an {\em overlay graph} $G(n, k, \delta, \gamma)$ as an arbitrary graph of $n$ nodes fulfilling the conditions of Theorem~\ref{theorem:overlay-graphs-exist}.
%Graph $G(n, k, \delta, \gamma)$ can be computed locally (i.e., in a single round) and deterministically by each process.
%Specifically, by Theorem~\ref{theorem:overlay-graphs-exist}, 
%the class of graphs satisfying the four properties (i) - (iv) is large, therefore any deterministic search in the class of $n$-node graphs, applied locally by each process, returns the same overlay graph $G(n, k, \delta, \gamma)$ in all processes.\footnote{%
%Recall that each round contributes~$1$ to the time complexity, no matter of the length of {\em local} computation.}

The next lemma shows that small subgraphs of a graph $G(n ,y)$ enjoys good connectivity properties. Let us define two meta-parameters $\delta = \frac{2}{3}y\ell, \gamma := \log{n} / \log{\delta}$.
\begin{lemma}[\cite{CK-PODC09}]\label{lemma:dense-are-big}		
If a graph $G$ is $(\ell,\frac{1}{3}y\ell,\frac{2}{3}y\ell)$-edge-dense, then any  $(\gamma,\delta)$-dense-neighborhood of a node $v\in V$ has at least $\ell$~nodes.
\end{lemma}

%\begin{lemma}
%\label{lemma:survival-small-diameter}	
%In a graph~$G(d)$ of $n$ nodes is
%$(\frac{k}{64})$-expanding, 
%$(\frac{k}{64},\frac{\delta}{8},\frac{\delta}{4})$-edge-dense
%and $(k,\frac{3}{4},\delta)$-compact, 
%then for any set $B\subseteq V$ of at least $k$ nodes and for any two nodes $v,w$ from set $C$ being a survival set of $B$, the nodes $v,w$ are of distance at most $2\gamma + 1$ in graph $G_{|C}$, for any $\gamma\ge 2\lg n$. 
%\end{lemma}


%\Paragraph{The new property.}

%The key new property of overlay graphs with good expansion, edge-\-density and compactness is that survival sets 
%(see compactness) 
%in such graphs~have~small~diameters.
%\BB




==> src/proofs-coin.tex <==
\section{Omitted proofs from Section~\ref{sec:quantum-coin}}\label{sec:coin-analysis}
\begin{proof}[Proof of Lemma~\ref{lem:surviving-probing}]
Consider two last iterations of the epoch $i$. Since the variable $\texttt{degree}_{p}$ has not changed it the epoch, thus also the variable $\texttt{adaptive\_degree}_{p}$ has remained unchanged in the epoch. In particular, examining line~\ref{line:while} assures, that in the last two testing rounds of this epoch, process $p$ received at least $\delta_{\alpha}$ responses from processes that had the variable $\texttt{adaptive\_degree}$ at least $\texttt{degree}_{p}$. 

Next, we proceed by induction. We claim, that in the $2j$ and $2j - 1$, for $1 \le j \le \gamma_{\alpha}$ last testing rounds there existed $(j, \delta_{\alpha})$-dense-neighborhood of $p$ with the properties the every processes belonging to this neighborhood is non-faulty and has its variable $\texttt{adaptive\_degree}$ at least $\texttt{adaptive\_degree}_{p}$. The induction step goes as follows. Assume that there exists $(j, \delta_{\alpha})$-dense-neighborhood of $p$ with the mentioned properties. In particular in the $2(j+1), 2(j+1) - 1$ last testing rounds, every process from this set had to receive at least $\delta_{\alpha}$ responses from processes with the variable $\texttt{adaptive\_degree}$ at least as big as the variable \texttt{adaptive\_degree} of the process. This follow from inspecting line~\ref{line:while}. The set of processes who responded with large values of \texttt{adaptive\_degree} constitute to the set $N^{j + 1}(p)$.

Eventually, we obtain the existence of the set $N^{\gamma_{\alpha}}(p)$ which satisfies the property of $(\gamma_{\alpha}, \delta_{\alpha})$-dense-neighborhood. Each process from the neighborhood has the variable $\texttt{degree}$ at least $\texttt{degree}_{p}$, since for every process $q$ it holds that $\texttt{degree}_{q} \ge \texttt{adaptive\_degree}_{q}$.
\end{proof}

\begin{proof}[Proof of Lemma~\ref{lemma:small-sets}]
Assume to the contrary that there exists an epoch such that more than $\frac{16n}{3\alpha^{i-2}}$ processes start this epoch with the variable $\texttt{degree}$ set to a value greater than $d\alpha^{i}$. Assume also w.l.o.g. that $i$ is the \emph{first} such epoch and let $A$ be the set of processes that have the variable $\texttt{degree}$ set to at least $d\alpha^{i}$ at the beginning of this epoch. Let $C$ be any survival set for $A$ with respect to the graph $\mathcal{G}(d\alpha^{i - 1})$. Note that since $A$ is a set of processes that are correct in epoch $i$, thus the processes from $C$ have been behaving correctly in epoch $1, \ldots, i -1 $ inclusively. Since the graph $\mathcal{G}(d\alpha^{i - 1})$ is $(16\frac{n}{d\alpha^{i - 2}},3/4,\frac{2}{3}\alpha)$-compact and $|A| \ge 16\frac{n}{d\alpha^{i - 2}}$, thus $C$ exists. At the beginning of the epoch $i$, the variable $\texttt{degree}$ of all processes from $C$ is greater than $d\alpha^{i}$, thus there must be a round $j < i$ in which the last process from $C$, say $q$, increases its variable $\texttt{degree}$ to $d\alpha^{i}$. But this gives us the contradiction. In the epoch $j$, all processes from $C$ operates in the graph $\mathcal{G}(d\alpha^{i - 1})$, thus they have at least $\delta_{\alpha}$ neighbors in $C$. All these neighbors have the variable $\texttt{degree}$ greater than $d\alpha^{i-1}$. In particular, in this epoch, the process $q$ will not execute line~\ref{line:if} and therefore it will not increase its variable $\texttt{degree}_{p}$ which give a contradiction with the maximality of $j$ and in consequence the minimality of $i$.
\end{proof}


Note that in the above proof of Lemma~\ref{lemma:small-sets} we use the fact that a suitable set $C$ of processes that have been correct throughout the whole epoch exists. We may choose this set and argue about it after the epoch, as the communication pattern in the algorithm is deterministic. Hence, in any round of the epoch,  processes in $C$ have at least as many non-faulty neighbors in communication graph as they have neighbors from set $C$. We use this number of neighbors in $C$ as a {\em lower bound} to argue about behavior of variables $\texttt{degree}$; therefore, our arguments do not depend on behavior of processes outside of $C$ and whether/when some of them fail during the epoch.

\begin{lemma}\label{lemma:non-faulty-ent}
Any two non-faulty processes $p$ and $q$ were connected by a quantum path of communication during the run of the algorithm. 
\end{lemma}
\begin{proof}
First observe, that the variable $\texttt{degree}_{p}$ can take at most $k + 1$ different values. Since there is $(k + 2)^{2}$ epochs, thus by the pigeonhole principle there must be a sequence of consecutive $k + 2$ epochs in which the variable $\texttt{degree}_{p}$ remains unchanged. Similarly, among these $k + 2$ epochs there must be two epochs in which the variable $\texttt{degree}_{q}$ remains unchanged. Let us denote these two epochs $i$ and $i + 1$. Since the variable $\texttt{degree}_{p}$ has not changed in the epoch $i + 1$, thus by applying Lemma~\ref{lem:surviving-probing}, we get that there exists a $(\gamma_{\alpha}, \delta_{\alpha})$-dense-neighborhood of $p$ in the graph $\mathcal{G}(\texttt{degree}_{p})$, say $A$, consisting of processes that a) were non-faulty in the epoch b) their variable $\texttt{degree}$ were at least $\texttt{degree}_{p}$. An immediate consequence is that all processes from $A$ were non-faulty in the epoch $i$. Moreover, since $A$ is $(\gamma_{\alpha}, \delta_{\alpha})$-dense-neighborhood of $p$ in the graph $\mathcal{G}(\texttt{degree}_{p})$ thus its size is at least $\frac{n\alpha}{\texttt{degree}_{p}}$ (Lemma~1~\cite{CK-PODC09}). Let $B$ be the analogues $(\gamma_{\alpha}, \delta_{\alpha})$-dense-neighborhood of $q$ derived from the properties of the graph $\mathcal{G}(\texttt{degree}_{q})$.


Now, consider quantum communication between sets $A$ and $B$ in the first testing round of the epoch $i + 1$. Processes from $A$ use the graph $\mathcal{G}(\texttt{degree}_{p})$ to communicate (or a denser graph) while processes from $B$ use the graph $\mathcal{G}(\texttt{degree}_{q})$ (or a denser graph). The graph $\mathcal{G}(\texttt{degree}_{p})$ is $(\frac{n\alpha}{\texttt{degree}_{p}})$-expanding and the graph $\mathcal{G}(\texttt{degree}_{q})$ is at least $(\frac{n\alpha}{\texttt{degree}_{q}})$-expanding. Therefore, at least one process from set $A$ inquires a process from set $B$ when executes line~\ref{line:inquires} in this testing round if $\texttt{degree}_{p} \ge \texttt{degree}_{q}$; or vice-versa if $\texttt{degree}_{p} < \texttt{degree}_{q}$. Since the set $B$ has diameter $\gamma_{\alpha}$ (Lemma~1~\cite{CK-PODC09}) and there remains $\gamma_{\alpha}$ testing rounds in the epoch $i +1$, thus by the end of this epoch any quantum messages send from $p$ could reach $q$.
\end{proof}

\begin{proof}[Proof of Theorem~\ref{thm:coin}]
Let $\mathcal{H} \subseteq \mathcal{P}$ be the set of initially non-faulty processes. Assume that at least $\frac{2}{3}|\mathcal{H}|$ of them remains non-faulty during the execution of the algorithm. By Lemma~\ref{lemma:non-faulty-ent}, any pair of processes from $\mathcal{H}$ is connected by quantum communication, therefore applying Lemma~\ref{lem:chance-win} to this set, gives that there is at least $\frac{2}{3} - o(1)$ (which is greater than $\frac{1}{2}$ for sufficiently large n) probability that all non-faulty processes return the same output bit. Since $0$ and $1$ are equally likely, thus the probabilistic guarantee on the weak global coin follows.
 
%Consider now the measurement in line~\ref{line:measurement} executed by any non-faulty processes which collapses all states entangled with this process. First, by a simply concentration argument, all entangled states with the process will collapse to different integers numbers in the range $[1, \ldots, x^{3}]$ whp. Second, there is at least $\frac{2}{3}$ chance that the maximum of these number will be assigned to a non-faulty process $q$ since the ratio of non-faulty processes to initially active processes is $\frac{2}{3}$ at least. In this scenario, all other non-faulty processes will output the measured quantum state $\ket{Coin_{q}}$ which has $\frac{1}{2}$ probability to be either $0$ or $1$. 
The number of rounds is deterministic and upper bounded by $O(k^2 \cdot \gamma_{\alpha}) = O\Big( \big(\frac{\log(n / d)}{\log{\alpha}}\big)^{2} \frac{\log{n}}{\log{\alpha}} \Big) = O\Big( \big(\frac{\log{n} }{\log{\alpha}}\big)^{3}\Big)$. To bound the communication complexity, assume that each graph $\mathcal{G}(d\alpha^{i})$, for $0 \le i \le k$, satisfies the desired expanding properties listed in the description of the algorithm. This, by the union bound argument, holds whp. By Lemma~\ref{lemma:small-sets} at the beginning of each epoch there is at most $\frac{16n}{d\alpha^{i - 2}}$ processes that inquires more than $d\alpha^{i}$ other processes in testing rounds of this epoch, for each $0 \le i \le k$. Since each message uses at most $O(\log{n})$ bits and qubits, thus a single testing round in an epoch adds at most
$$\sum_{i = 0}^{k} \frac{16n}{d\alpha^{i - 2}} \cdot d\alpha^{i} \le 16kd\alpha^{2} \cdot n\log{n}$$
qubits and bits to communication complexity. Since there is exactly $O\Big( \big(\frac{\log{n} }{\log{\alpha}}\big)^{3}\Big)$ testing rounds, thus the $O\Big( \big(\frac{\log{n} }{\log{\alpha}}\big)^{4}d\alpha^{2} \cdot n\log{n}\Big)$ upper bound on the total communication complexity of the algorithm follows. Dividing the latter by $n$ we receive amortized formula per process. %
\end{proof}


==> src/quantum-coin-proofs.tex <==
\section{The Analysis of \textsc{CheapQuantumCoin} Algorithm}
\label{sec:coin-analysis}




%\section{Why the approach of Chlebus, Kowalski and Strojnowski for $t < n$ does not work.}
%In paper~\cite{ChlebusKS10}, Chlebus, Kowalski and Strojnowski proposed a quantum algorithm that solves Consensus with probability at least $\frac{1}{2}$ in presence of arbitrary number $t < n$ of crashes. However, we suspect that there might be a flaw in their correctness argument. Using the terminology from their paper, in Lemma~7 they argue that the ticket of every non-faulty process $\p$ is delivered to every other non-faulty processes by the end of stage 3 of their algorithm even if $t < n$ crashes occurred. However, they do not argue how tickets of \textit{faulty} processes influence decisions of non-faulty processes. Usually, solving Consensus requires showing that every faulty processes is aware of the same subset of bits that come from faulty processes. They approach this issue by relaxing correctness condition to hold only with $\frac{1}{2}$ probability. This works well if the adversary can crash at most $\frac{1}{2}n$ all processes. In this case, with probability $\frac{1}{2}$ \textit{the largest} ticket is in possession of non-faulty process and is propagated among all non-faulty processes. However, this is no longer true if we allow arbitrary number of crashes. For instance the adversary can choose random $n - \sqrt{n}$ processes, partition them into $\sqrt{n}$ disjoint groups and crash them in such way that each non-faulty process gets information from different group of crashed processes. In this case, with probability $\frac{1}-\frac{1}{\sqrt{n}}$ the largest ticket will be delivered to only one of the non-faulty processes and the agreement will not hold.
\section{The Analysis of \textsc{FastCounting} Algorithm} %\label{sec:fast-counting-analysis}
Let us restate the theorem we prove in this section.
\begin{theorem}%[Section~\ref{sec:gossip-long}]
For any $2 \le x \le n$ and $\delta, \alpha \in \Omega(n)$, the \textsc{FastCounting} deterministic algorithm solves the 
%\Fuzzy 
fuzzy counting problem in $O\Big(\frac{\log{n}}{\log{x}}\big(\frac{\log{n}}{\log{\alpha}}\big)^{3}\Big)$ rounds, using $O\Big(x\frac{\log{n}}{\log{x}}\big(\frac{\log{n}}{\log{\alpha}}\big)^{4} d\alpha^{2}\log{n}\Big)$ (amortized) bits per process.
\end{theorem}
\begin{proof}
Let us first argue for the correctness. If $|\mathcal{P}| = 1$, then the conditional statement in line~\ref{line:base-case} proves the correctness. Next, we proceed by induction. Assume that the correctness is proved for any subset $\mathcal{P}' \subseteq \mathcal{P}$. Therefore, whenever a process $p$ executes a recursive call in line~\ref{line:recursive-counting}, its variable $\texttt{active}_{p}$ is assigned to the number being an estimation of non-faulty active processes in the set $\mathcal{P}_{g}$. Consider now set $\{ \texttt{active}_{p} : p \in \mathcal{P} \}$. This is the set of input messages to the execution of the Gossip algorithm, see line~\ref{line:fast-gossip}. Thus, by Theorem~\ref{thm:fast-gossip}, we get that unless all process from a group $\mathcal{P}_{p}$ crashes, then all other non-faulty processes will have the number $\texttt{active}_{p}$ in their sets $\mathcal{R}$ (line~\ref{line:fast-gossip}). Therefore, the sum returned in line~\ref{line:counting-output} is the actual estimate of the number of all-non faulty processes in the set $\mathcal{P}$, since it can differ from the number of all processes starting the algorithm only by the number of crashed processes.

The bounds on time and communication complexity follows immediately from the bounds on complexity of the Gossip algorithm proposed in Theorem~\ref{thm:fast-gossip} and the fact that depth of the recursion at most $O(\log{n} / \log{x})$.
\end{proof}
